Innovations Autoencoder and its Application in One-class Anomalous Sequence Detection

An innovations sequence of a time series is a sequence of independent and identically distributed random variables with which the original time series has a causal representation. The innovation at a time is statistically independent of the history of the time series. As such, it represents the new information contained at present but not in the past. Because of its simple probability structure, an innovations sequence is the most efficient signature of the original. Unlike the principle or independent component analysis representations, an innovations sequence preserves not only the complete statistical properties but also the temporal order of the original time series. An long-standing open problem is to find a computationally tractable way to extract an innovations sequence of non-Gaussian processes. This paper presents a deep learning approach, referred to as Innovations Autoencoder (IAE), that extracts innovations sequences using a causal convolutional neural network. An application of IAE to the one-class anomalous sequence detection problem with unknown anomaly and anomaly-free models is also presented.

==> figs/Structure+encoder.tex <==
%% Creator: Inkscape inkscape 0.92.5, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'Structure+encoder.eps' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{195.83893776bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.6057766)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength]{figs/Structure+encoder.eps}}%
    \put(0.01838246,0.24161361){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$\mathbf{x}_t$\end{tabular}}}}%
    \put(0.41828643,0.17267935){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$\hat{\nubf}_t$\end{tabular}}}}%
    \put(0.41828643,0.0761712){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$\mathbf{u}_t$\end{tabular}}}}%
    \put(0.64015535,0.21348217){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$\mathbf{D}_\gamma$\end{tabular}}}}%
    \put(0.85325203,0.19106153){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$W(\nubf_t,\mathbf{u}_t)$\end{tabular}}}}%
    \put(0.5951845,0.53880326){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$\mathbf{H}_\eta$\end{tabular}}}}%
    \put(0.21929676,0.24473505){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$\mathbf{G}_\theta$\end{tabular}}}}%
    \put(0.76377291,0.52612162){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$\hat{\mathbf{x}}_t$\end{tabular}}}}%
    \put(0.15931458,0.19106186){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Innovations \\Generator\end{tabular}}}}%
    \put(0.55300538,0.11446824){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Discriminator\end{tabular}}}}%
    \put(0.56066474,0.47752163){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Causal \\Decoder\end{tabular}}}}%
  \end{picture}%
\endgroup%


==> figs/viewgr.tex <==
%
%  vgmac.tex -- viewgraph macros for tex
%
%               vgmac is intended for use with the 12pt article style.
%               The commands currently suported are:
%               
%               Format commands:
%                  \horizfmt - horizontally formatted vg's
%                  \vertfmt  - vertically     "       "     (default)
%
%               Fonts:
%                  \bodyfont - std. font for body of vg     (default)
%                  \bodysmall - small font for body of vg
%                  \bodybold -  bold   "    "   "   "   "
%                  \bodyital - italic  "    "   "   "   "
%                  \titlefont - large font used for vg titles
%
%               Pagestyles:
%                  vgdatelabel - footer with left-justified filename
%                                and runtime, right-justified
%                                pagenumber                 (default)
%                  vgemptydatelabel - footer with left-justified runtime
%                                     and right-justified file name
%
%                 *N.B. if the filenames are relative to the current
%                       directory, the true path will appear in the footer
%                       only if the user has the following alias for latex:
%
%                       alias latex 'latex \\def\\dirname\{`pwd`\}\\input '
%
%               Page Initialization:
%                  \invg#1 - command to input a new viewgraph file.
%                            vg files are each assumed to contain a
%                            single vg.  #1 is as for the \input command.
%                  \newvgtitle#1 - command to initialize a vg with
%                                  title #1
%                  \newvgempty   - command to initialize a vg with no title
%
%                 *N.B. The first command in each vg file must be
%                       either \newvgtitle or \newvgempty
%
%               Text Layout:
%                  \leftitem#1 -      a bulleted, hanging indentation,
%                                     raggedright paragraph with contents #1
%                  \indentedpar#1#2 - a centered narrow paragraph #2
%                                     with bold label #1
%                  \bigskip -         has been redefined with infinite stretch
%
%                 *N.B. It is recommended that items in the viewgraph
%                       be seperated with \bigskip's
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  $Header: /user2/marcg/tex/macros/RCS/vgmac.tex,v 1.3 1992/02/11 01:20:42 marcg Exp marcg $
%
%  $Log: vgmac.tex,v $
%  Revision 1.3  1992/02/11  01:20:42  marcg
%  added \bodytiny and \bodytinyital
%
%  Revision 1.2  1991/03/19  01:10:40  marcg
%  added \par to \indentedpar
%
%  Revision 1.1  91/02/22  10:10:13  marcg
%  Initial revision
%  
%               
%  marcg, 1/22/91, Initial commented version
%  marcg, 1/29/91, Improved footer filename handling
%  marcg, 2/11/91, local definition of \xxvpt 
%  marcg, 2/20/91, changed def of indentedpar to use current value of 
%                  \textwidth
%  marcg, 2/21/91, replaced definition of \xxvpt with initialization
%                  of \@xxvpt for relative independence from
%                  lfonts.tex.  Dick mentioned that the rascals
%                  version of lfonts uses 25pt fonts in \xxvpt, while
%                  many other systems use 20pt fonts there.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\typeout{vgmac package, $Revision: 1.3 $, $Date: 1992/02/11 01:20:42 $}
%
% page layout and fonts 
%
\oddsidemargin -.25truein \topmargin -.25truein 
\headheight 0pt \headsep 0pt \topskip 0pt
\renewcommand\baselinestretch{1.1}
\def\magstepsix{2985}
\def\magstepseven{3583}
\font\titlefont = cmssbx10 scaled\magstep5
\font\bodyfont = cmss10 scaled\magstep4
\font\bodysmall = cmss10 scaled\magstep3
\font\bodytiny = cmss10 scaled\magstep2
\font\bodytinyital = cmssi10 scaled\magstep2
\font\bodybold = cmssbx10 scaled\magstep4
\font\bodyital = cmssi10 scaled\magstep4
\leftmargini .75 truein \rightmargin .5 truein
\leftmarginii .75 truein 
\leftmarginiii .75 truein
\leftmarginiv .75 truein
\itemsep 15pt plus 20pt minus 5pt
\def\bigskip{\vskip .9em plus 1fil minus .15em}
%
%  format comands
%
\def\horizfmt{\textwidth 9.50truein \textheight 7.0truein
\special{landscape}} 
%\special{header=/user/young/tex/macros/YMCAlandscapevglogo.ps}
\def\vertfmt{\textwidth 7.0truein \textheight 9.50truein}
%\special{header=/user/young/tex/macros/YMCAvglogo.ps} 
%
%  \newvgtitle starts a new titled viewgraph
%  \newvgempty starts a new untitled viewgraph
%
\def\newvgtitle#1{\begin{center} \Huge\titlefont #1 \\[-.2em]
\rule{\textwidth}{2pt}
\end{center}
\LARGE\bodyfont
\raggedright
\parindent 0pt
}
\def\newvgempty{\LARGE\bodyfont\raggedright\parindent 0pt}
%
%  \invg inputs a viewgraph file and sets up footer filename as
%  follows:
%     filename starting with '/' --> footer contains filename
%     otherwise --> footer contains filename prepended with \dirname
%                   if it exists.
%
\def\invg#1{\clearpage\def\vgfilename{#1}
  \getinit{#1}
  \gdef\vglabelname{%
    \if\initchar/\else%
      \expandafter\ifx\csname dirname\endcsname\relax%
      \else\expandafter\badBgone\dirname\relax/\fi\fi%
        \expandafter\badBgone\vgfilename\relax.tex}%
\input #1}
%
%  \getinit sets the global variable \initchar to the first token of
%  its argument.
%
\newif\ifreadone  % used by \firstchar
\def\getinit#1{\firstchar#1\relax}
\def\firstchar#1{%
  \ifreadone\relax\else \gdef\initchar{#1}\readonetrue\fi%
  \if #1\relax\readonefalse\let\next=\relax%
  \else\let\next=\firstchar\fi%
  \next%
}
%
%  \leftitem yields a left justified paragraph with a bullet
%
\def\leftitem#1{\medskip
\setbox1\hbox{$\bullet$\hskip 1em}
\leavevmode\hangindent\wd1\hangafter1{\box1 #1\par}}
%
%  \indentedpar yields an narrow centered paragraph, #2, with label #1
%  The idea is to make the lines of the parbox maximally long with
%  no hyphenation and a raggedright.  The argument of the parbox used
%  to be '\raggedright #2'
%
\newdimen\indparind\indparind 3em
\newdimen\indparwd
\long\def\indentedpar#1#2{\indparwd\textwidth\advance\indparwd by -2\indparind
  {\bodybold #1:}\hfil\break
  \null\hskip\indparind\parbox[t]{\indparwd}{%
\linepenalty 10000\hyphenpenalty 10000\rightskip 0pt plus3em{#2}}\par}
%
%  makeatletter required for badBgone, ps@vgdatelabel,
%  ps@vgemptydatelabel, xxvpt
%
\makeatletter
\def\badBgone#1{\toks0={#1}\expandafter\if\the\toks0\relax%
    \let\next=\relax\else%
    \expandafter\if\the\toks0_\_%
    \else\expandafter\if\the\toks0&\&%
    \else\expandafter\if\the\toks0$\$%
    \else\expandafter\if\the\toks0^\^{ }%
    \else\expandafter\if\the\toks0<$\m@th <$%
    \else\expandafter\if\the\toks0>$\m@th >$%
    \else\expandafter\if\the\toks0##{$\m@th\sharp$}%
    \else\expandafter\if\the\toks0\noexpand{{$\m@th\{$}%
    \else\expandafter\if\the\toks0\noexpand}{$\m@th\}$}%
    \else\expandafter\if\the\toks0\noexpand%\%%
    \else\the\toks0\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi%
    \let\next=\badBgone\fi%
    \next}%
%
%
\def\ps@vgdatelabel{\let\@mkboth\@gobbletwo
     \def\@oddhead{}
     \newdimen\mydimen \mydimen=\textwidth
     \divide\mydimen by 2
     \newcount\hours \hours=\time \divide\hours by 60
     \newcount\minutes \minutes=\hours \multiply\minutes by
                           -60 \advance\minutes by\time
     \def\@oddfoot{\hbox to\textwidth{\footnotesize\sl\today, \the\hours:%
         \ifnum\minutes<10 0\fi\the\minutes\ --- %
         \vglabelname\hfill\rm\thepage}}
     \def\@evenhead{}\let\@evenfoot\@oddfoot%
     }
%
%
\def\ps@vgemptydatelabel{\let\@mkboth\@gobbletwo
     \def\@oddhead{}
     \newdimen\mydimen \mydimen=\textwidth
     \divide\mydimen by 2
     \newcount\hours \hours=\time \divide\hours by 60
     \newcount\minutes \minutes=\hours \multiply\minutes by
                           -60 \advance\minutes by\time
     \def\@oddfoot{\hbox to\mydimen{\footnotesize\sl\today, \the\hours:%
         \ifnum\minutes<10 0\fi\the\minutes\hfill}\hss%
         \hbox to\mydimen{\quad\footnotesize\sl\hfill%
         \vglabelname\hss}}
     \def\@evenhead{}\let\@evenfoot\@oddfoot%
     }
%
%  xxvpt is called by \Huge at 12pt in article style, so we initialize
%  @xxvpt to load in sanserif fonts.  This allows us to override the 
%  definition in xxvpt independent of the machine type.  This whole
%  exercise is to fix some of my math macros that use \sf
%
%\@getfont\psf\sffam\@xxvpt{\@mss\@magscale5}\normalsize
\makeatother
%
%  default is vertical format and vgdatelabel pagestyle
%
\vertfmt
\pagestyle{vgdatelabel}



